On the adversarial robustness of Locality-Sensitive Hashing in Hamming space

Locality-sensitive hashing~[Indyk,Motwani'98] is a classical data structure for approximate nearest neighbor search. It allows, after a close to linear time preprocessing of the input dataset, to find an approximately nearest neighbor of any fixed query in sublinear time in the dataset size. The resulting data structure is randomized and succeeds with high probability for every fixed query. In many modern applications of nearest neighbor search the queries are chosen adaptively. In this paper, we study the robustness of the locality-sensitive hashing to adaptive queries in Hamming space. We present a simple adversary that can, under mild assumptions on the initial point set, provably find a query to the approximate near neighbor search data structure that the data structure fails on. Crucially, our adaptive algorithm finds the hard query exponentially faster than random sampling.

==> conclusion.tex <==
\section{Conclusions}

In this paper we have shown that it is in principle possible to attack standard LSH schemes and force false positives exponentially faster than it would be possible with non-adaptive queries. This underlines the importance of recent work on false-negative-free LSH \cite{P18,Ahle17,Wei22} as well as adversarial robustness \cite{BeimelKMNSS22,AttiasCSS23,CohenNSS23} and shows that more work is required in resource-restricted settings.


==> old.tex <==
\section{Violating external correctness for Hamming space LSH in constructed case.}

Here we use the construction\footnote{We set bucket size to $1$ as it is irrelevant for our purposes.} described in \cite{gionis1999similarity}.

\paragraph{Setting.}
Let $n, d$ be large enough, let $\delta \approx 1 / \poly n$ be the failure probability of a single query. Let $P$ be a set of $n$ points in $d$-dimensional Hamming space $H := \{0, 1\}^{d}$. Hash function set is defined as $\mathcal{H} = \{\forall i \in [d]: h_i(p) = p_i\}$.
Let $r_1 = d/10$, $r_2=d/5$, $p_1=1-r_1/d = 0.9$, $p_2 = 1 - r_2/d = 0.8$, $k = \log_{1/p_2} n \approx 3.1 \cdot \log n$, $\rho = \frac{\log 1/p_1}{\log 1/p_2} \approx 0.47$, $l = n^{\rho}$.
The structure consists of $l$ hash functions $g=\{h_1, \ldots, h_k\}$ chosen at random. It is repeated $\approx \log(1/\delta)$ times.
\xxx[MM]{I don't think we need to specify the constants.}

For a function $g$, let $G(q) = \{p \in P: g(p) = g(q)\}$. LSH only stores at most one point from $G(q)$ for each $q$, which we will denote $g^*(q)$. Hence instead of repeating the structure $\log(1/\delta)$ times we can just set $l = n^\rho \log(1/\delta)$.

\paragraph{Set construction.} We construct the set $P$ with $n=2^m$ as follows: let $z=(0, \ldots, 0)$, $P_1 = \{ (p'_1, \ldots, p'_m, 1 \ldots, 1) : \forall p' \in \{0, 1\}^m \setminus \{(0, \ldots, 0)\}\}$. Then $P = P_1 \cup \{ z \}$.

A crucial property of this set is that $z$ and $P_1$ never hash into the same bucket.
\begin{lemma}[No mixing] \label{lem:ham_no_mixing}
If $k > m$, then for any $q \in H$ and for any $g$, if $z \in G(q)$ then $G(q) = \{z\}$.
\end{lemma}
\begin{proof}
Assume $z \in G(q)$. Since $k > m$, there exists $i \in [k]$  such that $h_i$ in $g$ returns an entry with index greater than $m$. Since all points in $P_1$ are equal to $1$ on all of those indices, and $z$ is all zeros, $\forall p' \in P_1: g(z) \neq g(p')$, hence $G(q) \cap P_1 = \emptyset$ and $G(q) = \{ z\}$.
\end{proof}

This means that as long as we query inside the ball $B(z, r_2)$, violation of \Cref{prop:bad_coll} doesn't change the output of the datastructure.

\begin{corollary}
If $q \in B(z, r_2)$, LSH returns $z$ iff $z$ collides with $q$.
\end{corollary}
\begin{proof}
    Forward direction follows from construction. Reverse direction follows from \Cref{lem:ham_no_mixing}.
\end{proof}

\subsection{Algorithm}

The algorithms consist of an outside loop and a support recovery step run inside this loop. 

\paragraph{Recovery step} The purpose of the recovery step is to recover at least $k/2$ supporting bits of one of the functions $g$.

\begin{definition}
For a point $q \in H$, $Z(q)$ is the set of functions $g$ used by LSH that collide $q$ and $z$.
\end{definition}

Note that we cannot observe $Z(q)$ directly, we can only check whether it is empty for a $q \in B(z, r_2)$.

The estimation step takes as an input at most $O(d/k)$ fixed bits $T$.

First, we pick $q$ at such a distance $r'$ so that the expected size of $|Z(q)|$ is constant and all bits $T$ are equal to $1$. For that we need that
\[
    \left( 1 - \frac{r'}{d} \right)^{k} \leq n^{-\rho} \log( 1/ \delta)^{-1}.
\]
Hence $r' \geq c \cdot r_1 + (1 - c) \cdot d$, where $c = (\log 1/\delta)^{-1/k} = 2^{-\frac{\log \log 1/\delta \cdot \log 1/p_2}{\log n}}$. So for a large enough $n$, $r' \leq (r_1 + r_2)/2$.

We sample $q$ until we find one that collides with $z$.
\xxx[MM]{The distance to $q$  should actually be chosen adaptively based on the set $T$.}

We will maintain the set $S$ of bits that are supporting for all functions $Z(q)$. It starts empty. While the size of set $S$ is at most $k/2$ repeat the following.

Flip at random $d/k$ bits of $q$ that are equal to $0$ and don't lie in $S$ to get $q'$. Note that $\dist(q', z) \leq r_2$ if $n$ is sufficiently large.
Now, each function $g$ which collides $q$ and $z$ doesn't collide $q'$ and $z$ with constant probability. Hence with constant probability $z$ doesn't collide with $q'$.
We repeat sampling of $q'$ until we find one that does not collide with $z$.

% \xxx[MM]{We can just sample point $q'$ directly then binary search between it and $z$.}

Now we can perform binary search between $q$ and $q'$ by flipping half of the bits equal to one in $q' - q$ and adding it to $q$, then checking if that new point collides with $z$ or not.
We continue doing it until we find two points $q_1$ and $q_2$ such that $q_1$ collides with $z$ and $q_2$ doesn't and they are different in only $1$ bit --- let it be $i$.

We can now conclude that among the $O(1)$ functions in $Z(q)$, bit $i$ is a supporting bit for at least one of them. We now flip the bit $i$ in $q$ to get $q_3$. If $q_3$ still collides with $z$, then $i$ is not a supporting bit for all functions $Z(q)$ and $Z(q_3)$ is not empty. In this case we set $q := q_3$. Otherwise we leave $q$ unchanged and add $i$ to $S$. Then we continue to the next iteration.

Note that we don't move $q$ during the execution by distance more that $O(1)$.

\paragraph{Outer loop}
In the outer loop we maintain a set of partial supports $\mathcal{U} = \{S_i\}$, $|S_i| \geq k/2$. At each iteration we find a covering set $T$ such that $T \cap S_i \neq \emptyset$ for all $i$ greedily by iteratively adding to $T$ the bit that covers the most uncovered sets. This produces a set of size at most $2d/k$. \xxx[MM]{Should this be $d/k \cdot \log \ell$ instead? Maybe there is no $\log \ell$ w.h.p. if the $g$'s are picked uniformly.} Then we call the recovery step with set $T$ and add the returned set $S_i$ to $U$. When $|U| = \ell$, we find the set $T$ again, and the query where all bits of $T$ are equal to $1$ would not collide with $z$ while being inside radius $r_1$, which would violate the LSH correctness.

==> old2.tex <==
We are now ready to analyze \cref{alg:simple}.

\begin{restatable}[Simplest algorithm]{theorem}{simple} \label{thm:simple}
Let $n>e$, $28 \ln^3 n \leq r \leq d/(28 \ln n)$, $\lambda \leq \frac{1}{8e^2} \min\{\frac{r}{\ln n}, n^{1/8}\} - 1$, and $1 + \frac{80 + 16 \ln(\lambda + 1)}{\ln n} \leq c \leq \ln n$.
%Let $n > e$ and
%\begin{itemize}
%    \item $28 \ln^3 n \leq r \leq d/(28 \ln n)$,
%    \item $\lambda \leq \frac{1}{8e^2} \min\{\frac{r}{\ln n}, n^{1/8}\} - 1$,
%    \item $1 + \frac{80 + 16 \ln(\lambda + 1)}{\ln n} \leq c \leq \ln n$.
%\end{itemize}
Let $t = 2e^2 (\lambda + 1)$ be the parameter from \cref{alg:simple}. Suppose that the point $z$  passed to \cref{alg:simple} is located at a distance of at least $2cr$ from any other point in $P$. With probability at least $1/4 - 1/n$ the algorithm finds a point $q$ at a distance of at most $r$ from $z$ such that querying LSH with $q$ returns no point. It uses at most $O(cr \cdot \lambda)$ queries to the LSH data structure.
\end{restatable}

Here we present only the conceptual part of the proof of \cref{thm:simple}. 
The full proof can be found in \cref{app:simple_analysis}

\begin{proof}[Proof outline]
Let $q_i$ be the value of $q$ at the end of the iteration $i$ inner loop of \cref{lem:simple_inner_loop}, and let $q_0$ be its value at the beginning of the first iteration of this loop. Let $i^*$ be the number of iterations.

For each iteration $i$ of the inner loop, by \cref{lem:simple_inner_loop} two points $q'$ and $q''$ are found. The bit where they differ must lie in the support of one of the hash functions in $\coll(q'', z)$ since $\lsh(q') \neq z$. Since $q_i$ and $q_{i-1}$ differ in only this bit, and because $\coll(q', z) \subseteq \coll(q_{i-1}, z)$, it holds that $|\coll(q_i, z)| < |\coll(q_{i - 1}, z)|$, so the size of the $|\coll(q_i, z)|$ decreases by at least $1$ after each execution of the loop. {\bf MK: $i$  not defined}

By \cref{lem:near_coll} and Markov's inequality, $|\coll(q_0, z)|$ is at most $2e^2(\lambda + 1)$ with constant probability, so at most $2e^2 (\lambda + 1)$ iterations will be made until $\coll(q_{i^*}, z) = \emptyset$, which also means that $\lsh(q_{i^*}) = \bot$ so the loop stops. On the other hand, $\dist(q_{i^*}, z) \leq r$, which makes $q_{i^*}$ a false negative query. {\bf MK: $i^*$ not defined.}
\end{proof}


% \paragraph{Discussion of parameter bounds}
% \xxx[MM]{TODO: finish}
% \[
% \lambda \leq \frac{1}{8e^2} \min\left\{\frac{r}{\ln n}, n^{1/8}\right\} - 1
% \]
% This is essentially two upper bounds on $\lambda$, in terms of $r$ and $n$.
% Note that by union bound, if $\lambda \geq O(r \log d \poly \log n) \geq \log \binom{d}{r} \cdot O(\poly \log n)$, with high probability the structure correctly answers all queries within the distance $r$ of any point in the dataset, meaning that it never produces a wrong answer. Hence our upper bound in $r$ is tight up to polylogarithmic factors.
% The upper bound of $O(n^{1/8})$ well covers the typical range of $\lambda$, as it is usually set to be $O(\poly \log n)$.

% \xxx[MM]{Not sure what to say about the rest.}

\subsection{The fast algorithm} \label{sec:fast_alg_analysis}
With a simple modification of the inner loop of \cref{alg:simple}, we can exponentially reduce the dependence on $r$ in the running time and the number of queries. 
% Since the algorithm gets only one bit of information from each query, this means it only requires the amount of information roughly equal to the size of $\lambda$ indices encoding a position in a $d$-dimensional vector to construct a failing query. \xxx[MK]{I am unable to parse this last sentence.}

We state the algorithm and give the proof of its correctness in \cref{sec:fast_analysis}. On a high level, instead of using a linear search as in \cref{alg:simple} to find a pair of points $q''$, $q'$ such that $\coll(q'', z) \neq \emptyset$ and $\coll(q', z) = \emptyset$, we use a binary search in the inner loop. We still start with the same point $q$. However, we now flip the $cr - \dist(q,z)$ bits in $q$ in positions where $q$ equals $z$ to get $q^{(r)}$. Then by \cref{lem:far_coll}, $q^{(r)}$ does not hash with $z$. Now we use a binary search on the path from $q$ to $q^{(r)}$ to find the aforementioned pair of points. The analysis is analogous to that of \cref{lem:simple_inner_loop}.

\begin{restatable}[Faster algorithm]{theorem}{fast} \label{thm:fast}
Let $n > e$ and
\begin{itemize}
    \item $28 \ln^3 n \leq r \leq d/(28 \ln n)$,
    \item $\lambda \leq \frac{1}{8e^2} \min\{\frac{r}{\ln n}, n^{1/8}\} - 1$,
    \item $1 + \frac{80 + 16 \ln(\lambda + 1)}{\ln n} \leq c \leq \ln n$.
\end{itemize}
Let $t = 2e^2 (\lambda + 1)$ be the parameter from \cref{alg:fast}. Suppose that the point $z$  passed to \cref{alg:fast} is located at a distance of at least $2cr$ from any other point in $P$. With probability at least $1/4 - 1/n$ the algorithm finds a point $q$ at a distance of at most $r$ from $z$ such that querying LSH with $q$ returns no point.
It uses at most $O(\log (cr) \cdot \lambda)$ queries to the LSH data structure.
\end{restatable}

